"Kurosawa": A Script Writer's Assistant

Storytelling is the lifeline of the entertainment industry -- movies, TV shows, and stand-up comedies, all need stories. A good and gripping script is the lifeline of storytelling and demands creativity and resource investment. Good scriptwriters are rare to find and often work under severe time pressure. Consequently, entertainment media are actively looking for automation. In this paper, we present an AI-based script-writing workbench called KUROSAWA which addresses the tasks of plot generation and script generation. Plot generation aims to generate a coherent and creative plot (600-800 words) given a prompt (15-40 words). Script generation, on the other hand, generates a scene (200-500 words) in a screenplay format from a brief description (15-40 words). Kurosawa needs data to train. We use a 4-act structure of storytelling to annotate the plot dataset manually. We create a dataset of 1000 manually annotated plots and their corresponding prompts/storylines and a gold-standard dataset of 1000 scenes with four main elements -- scene headings, action lines, dialogues, and character names -- tagged individually. We fine-tune GPT-3 with the above datasets to generate plots and scenes. These plots and scenes are first evaluated and then used by the scriptwriters of a large and famous media platform ErosNow. We release the annotated datasets and the models trained on these datasets as a working benchmark for automatic movie plot and script generation.

==> Sections/5_Background.tex <==
\section{Background and Terminologies}
\label{sec4}
In this section, we will explore the structure of a screenplay and some story templates in detail.

\subsection{Screenplay}
\label{subsec:screenplay}
A movie script or a screenplay has a different format than a story. A script is a group of scenes. Each of these scenes consists of a few major components, which are discussed below: 

\textbf{Scene Headings/Sluglines}--- This component describes the when and where of the scene. It can be thought of as the first shot that a camera takes of a new scene. For example, INT. - RESTAURANT - NIGHT indicates that the scene starts inside a restaurant at night. Sluglines are normally written in capital letters and are left-aligned.

\textbf{Character Names}--- They are mentioned every time a character is going to speak dialogue. The name of each character is mentioned in uppercase and is centre aligned.

\textbf{Dialogues}--- Dialogues are the lines that the characters say. They appear right after the character name in a script and are centrally aligned.

\textbf{Action Lines} --- Action lines describe almost everything about a scene. They can be described as the narration of each script. Action lines can be present either after dialogues or sluglines and are left-aligned.

\textbf{Transitions} --- A transition marks the change from one scene to the next. They also depict how a scene is ended. For example, DISSOLVE, FADE, and CUT are different keywords used to indicate a transition. They are usually in upper case and are right-aligned. 

Figure \ref{fig:screenplay} shows an example of the screenplay elements.

\begin{figure}[h]
    \centering
    \fbox{\includegraphics[width=0.95\columnwidth]{Images/screenplay_elements_new.png}}
    \caption{The elements of a screenplay}
    \label{fig:screenplay}
\end{figure}

\subsection{Story Templates}
\label{subsec:actdivision}

%Storytelling has been prevalent as a means of human communication for thousands of years
Over time there have been developed various templates that help to create stories. One of the most famous templates is the 3-act structure \cite{field1979screenplay}. This structure divides a story into a \textit{setup, confrontation and resolution}. We will now look at the 4-act structure in detail, an extension of the 3-act structure.

\textbf{Act 1}--- This is the opening/introduction act. It describes the protagonist's character and briefly introduces the movie's theme. The act ends with the start of a new journey for the protagonist.

\textbf{Act 2A}--- Due to the vast span of Act 2, it can be divided into two acts. This act usually contains the start of a love story. It also entertains the audience as the protagonist tries to adapt to their new journey. The act ends as the movie's midpoint, one of the film's critical moments, with either a very positive or negative scene.
    
\textbf{Act 2B}--- This act usually contains the protagonist's downfall. The villain or antagonist starts to gain an advantage, and the protagonist loses something or someone significant. The act ends with the protagonist realizing their new mission after reaching rock bottom.

\textbf{Act 3}--- The protagonist has realized the change required in them and sets out to defeat the antagonist in a thrilling finale. The movie then ends by displaying a difference in the protagonist that was lacking in the beginning.
